A Self-explaining Neural Architecture for Generalizable Concept Learning

With the wide proliferation of Deep Neural Networks in high-stake applications, there is a growing demand for explainability behind their decision-making process. Concept learning models attempt to learn high-level 'concepts' - abstract entities that align with human understanding, and thus provide interpretability to DNN architectures. However, in this paper, we demonstrate that present SOTA concept learning approaches suffer from two major problems - lack of concept fidelity wherein the models fail to learn consistent concepts among similar classes and limited concept interoperability wherein the models fail to generalize learned concepts to new domains for the same task. Keeping these in mind, we propose a novel self-explaining architecture for concept learning across domains which - i) incorporates a new concept saliency network for representative concept selection, ii) utilizes contrastive learning to capture representative domain invariant concepts, and iii) uses a novel prototype-based concept grounding regularization to improve concept alignment across domains. We demonstrate the efficacy of our proposed approach over current SOTA concept learning approaches on four widely used real-world datasets. Empirical results show that our method improves both concept fidelity measured through concept overlap and concept interoperability measured through domain adaptation performance.

==> 3_method-old.tex <==
\section{Methodology}
\label{sec:method}
We now describe our two-step semi-supervised concept learning (SSCL) framework. Figure~\ref{fig:schematic-diag} shows the overall pipeline of SSCL, which consists of a semi-supervised robust concept extraction module and followed by a supervised concept alignment module. 
%\jianhui{Can you name our proposed model using some short form so that we could easily refer to it? Now it is super difficult to call the full name. "SSCE" is only the short form of a part of the model, not the entire one}



% SENN consists of two networks - $h$ and $\theta$, where $h$ learns interpretable concepts, while $\theta$ learns the corresponding relevance scores. During training, each sample is passed through both $h$ and $\theta$ to generate concept representations and relevance scores respectively. The premise behind this approach is that concepts form a basis of the latent space and a combination of concepts is utilized to perform the prediction task. Representations and scores are combined using a third network (aggregator) $g$ which combines concepts and relevance scores to perform the final prediction.



\subsection{Semi-supervised Concept Extraction (SSCE)}
\label{sec:hp-ssce}
%\jianhui{rewrite this in a high level}
In this section, we introduce Semi-Supervised Concept Extraction (SSCE) which leverages contrastive learning to extract robust and generalizable concepts. We recognize that the concepts learned from existing approaches fail to generalize to even similar domains because of two reasons. First, the concept learning process is sensitive to even slight data transformation and distributional shift. Second, the extracted concepts cannot even guarantee concept sharing among samples belonging to same class due to a lack of class label supervision.

In Section~\ref{sec:SS-CSS}, we propose to use self-supervised learning to improve the robustness to common data transformations. Specifically, we curate tuples of positive and negative samples, which are samples under small and large transformations, respectively. We subsequently enforce concepts learned from positive samples to be similar while concepts learned from negative samples to be dissimilar. In Section~\ref{subsec:semi}, we propose to regularize the disparity between concepts learned from data instances among same classes. We then in Section~\ref{subsec:end-to-end} explain how all pieces combined is able to extract generalizable concepts.


% To address concept interoperability, we first propose a self-supervised training paradigm to smoothen the concept space. The training paradigm includes construction of positive and negative samples which in pair computes a contrastive loss. Positive sampling is able to improve 
% robustness of concepts\cite{lee2022self}, while negative sampling enforces domain invariance. Further, concepts from the same class are constrained using semi-supervised concept parity to avoid divergence between representations of concepts from the same class which is attested firmly by our empirical results in Section~\ref{sec:intraoverlap}. Next, we provide details of the pretext tasks considered in self-supervised smoothing. %\jianhui{In Section~\ref{subsec:semi}, we provide details of the pretext tasks considered in self-supervised smoothing which (summarize the design objective here)} 
% Further, we discuss the constraints enforced in the form of concept parity. %Finally, we conclude by demonstrating how concept codes are utilized in supervised concept alignment training. 

%\textbf{Overview:} As discussed in Section~\ref{sec:intero}, it is important to both improve robustness and isolate 
% \jianhui{isolate is inaccurate, maybe disentangle} 
%Basically, you have to use one sentence to describe what is positive sampling before you explain what they are used for.}  
% \jianhui{"This module is capable of doing xxx, which is attested firmly by our empirical results." Basically, the original sentence stops too abruptly and does not reveal the outcome of this module, which is necessary for a summarization.}

\subsubsection{Self-Supervised Concept Space Smoothing (CSS)}
\label{sec:SS-CSS}
In recognition of existing concept learning approaches which struggle to generate concepts robust to data transformations, we propose to apply contrastive learning to prepare the concept learning process with possible distribution shift. We call this novel technique as Self-Supervised Concept Space Smoothing (SS-CSS). The general idea is we deliberately generate similar and dissimilar data instances with the goal to diversify and smoothen the concept distribution such that the extracted concepts are able to be less sensitive to common distributional shift.

Specifically, we propose to utilize a modified version of contrastive loss\cite{wang2021understanding} for self-supervised learning\cite{oord2018representation}. For a given data point $x$ (anchor), we generate two other sets of data points - a positive set $X^{+}$ and a negative set $X^{-}$. For a given concept encoder network $f_e$, the embedding of a data point $x$ in the concept space is represented as $f_e(x)$ and $s(f_e(x_i), f_e(x_j))$ represents a similarity measurement between two data points $x_i$ and $x_j$'s concept representation, where the similarity metric selection is task-specific. Note that in Figure~\ref{fig:schematic-diag}, the encoder $f_e$ during inference is represented as $g$.
%Self-supervised concept training paradigm enables automatic concept extraction as concepts are relatively robust entities and remain invariant to small input space transformations. However, large transformations may change the inherent structure of the object in question resulting in low concept similarity. 
%\jianhui{delete "even though domain is still constant" as it is obvious since you are only operating on a single data point}. 
%To this effect, we propose to utilize a modified version of contrastive loss\cite{wang2021understanding} for self-supervised learning\cite{oord2018representation}. For a given data point $x$ (anchor), we generate two other sets of data points - a positive set $X^{+}$ and a negative set $X^{-}$. For a given concept encoder network $f_e$, the embedding of a data point $x$ in the concept space is represented as $f_e(x)$ and $s(f_e(x_i), f_e(x_j))$ represents a similarity metric between two data points $x_i$ and $x_j$'s concept representation, where the metric selection is task-specific.
% \jianhui{", where the metric selection is task-specific."}. 

The objective of contrastive loss maximizes the similarity between an anchor image $x$ and set of positive samples $X^{+}$  while simultaneously minimizes the similarity between anchor and negative samples $X^{-}$. The extent of similarity is adjusted using a tunable hyperparameter $\tau$ (\textit{temperature}), which controls the penalty on both positive and negative samples. Formally, the self-supervised loss $\mathcal{L}_{SSL}$ parameterized by anchor (x), positive sample ($x^+$) and negative sample ($x^-$), can  be formulated as Equation~\ref{eq:ssl}.
% \begin{equation}
%     \label{eq:ssl}
%     \mathcal{L_{SSL}} = -\log (\frac{\Sigma_{x^+ \in X^+}\text{exp}(s(x,x^+)/\tau)}{ \Sigma_{x^- \in X^-}\text{exp}(s(x,x^-)/{\tau})+\Sigma_{x^+ \in X^+}\text{exp}(s(x,x^+)/{\tau}))}) 
% \end{equation}
\begin{equation}
    \label{eq:ssl}
    \mathcal{L_{SSL}}= -\log (\frac{\text{exp}(s(e,e^+)/\tau)}{\text{exp}(s(e,e^-)/{\tau})+\text{exp}(s(e,e^+)/{\tau}))}) 
\end{equation}
where we use $e\triangleq f_e(x)$, $e^+\triangleq f_e(x^+)$, $e^-\triangleq f_e(x^-)$ to represent the embedding of anchor, positive sample, and negative sample, respectively.

%% Re-write this paragraph to include the newer ssl
To generate $X^+$ and $X^-$, we follow two commonly used approaches - crop/rotate and SimCLR, discussed in more detail Section~\ref{sec:ssl-choice}. Both approaches entail creating a positive set of samples by performing small transformations while the negative set is generated with bigger transformations. We utilize \cite{xu2019self} for crop/rotation while the SimCLR approach is used from \cite{chen2020simple}.
% Positive samples ($X^+$) are generated for a given anchor $x$ as images by small rotations and random cropping transformations. We utilize \cite{xu2019self} strategy to generate harder samples by creating higher rotation transformations. 
Visually, the sampling procedure, more details on the choice of contrastive learning and the associated loss function are provided in the Appendix.
% Figure~\ref{fig:sampling-diag} (Appendix). 



\subsubsection{Semi-Supervised Concept Parity (SSCP)}
\label{subsec:semi}
Although SS-CSS described is able to robustify concepts against common data transformations, there is still no guarantee for concept consistency for data from the same class. We call the property of concept sharing among data with same label as \textit{concept parity}. To achieve concept parity - we apply a constraint to enforce the similarity of concepts of data instances from the same label class. Formally,
\begin{equation}\label{eq:parity}
    \mathcal{L}_{parity} = l(f_e(x_i),f_e(x_j))~~~\text{for}~~ y_i = y_j
\end{equation}
where $l (\cdot, \cdot)$ is a customized similarity measure which may not equal to $s$ in Equation~\ref{eq:ssl} and $f_e(\cdot)$ is a mapping function from the input space to the concept space, while $y$ is the label for each data instance.

\subsubsection{End-to-end Training Using SSCE}
\label{subsec:end-to-end}
For a given encoder network $f_e$ mapping inputs to the concept space, we define a decoder network $f_d$ 
% \jianhui{how about using $f_e$ as encoder and $f_d$ as decoder, currently, the notation of $f$ and $f'$ is confusing} 
which maps from the concept space to the input space. For a given sample $x_i$, its concept embedding is defined as $f_e(x)$ and reconstruction is defined as $f_d(f_e(x))$. Finally, to increase diversity among concepts, sparsity is enforced by regularizing $f_e(x)$. Formally,
\begin{equation}\label{eq:sparsity}
    \mathcal{L}_f = l(x, f_d(f_e(x))) + \lambda*||f_e(x)||_{1} 
\end{equation}

\noindent where $\lambda$ is a tunable hyperparameter which controls the strength of the sparsity constraint. For implementation details on sparsity constraint imposed upon matrix-valued data, please refer to Section~\ref{sec:setup}.

\\
\vskip 15pt
\noindent Putting all the pieces together we have the following training objective for SSCE:
% \jianhui{the word "final SSCE training objective" is not very formal, can be better written as "putting all pieces together, we have the following training objective for SSCE"} can be written mathematically as:
\begin{equation}\label{eq:end-to-end}
    \mathcal{L}_{SSCE} = \mathcal{L}_f  + \alpha*\mathcal{L}_{SSL} + \beta*\mathcal{L}_{parity}
\end{equation}

% \jianhui{define L1 sparsity regularization, you can say "details could be found in experiment section" if you do not want to go into details, but you cannot go without definition.}

\noindent where $\alpha$ and $\beta$ are tunable hyperparameters. We find the results are insensitive and any reasonable selection of hyperparameters achieve satisfactory results. 
We defer the pseudocode of SSCE to Appendix.
% \jianhui{Please write one more sentence summarizing the sensitivity of these hyperparameters after the experimental section is done.}


\subsection{Supervised Concept Alignment (SCA)}
\label{sec:sca}

We now introduce the second module of SSCL, Supervised Concept Alignment (SCA), which aims to leverage domain-invariant and robust concepts generated with SSCE in the source domain as supervision to help generate concepts that are capable to generalize well to target domains. 

\subsubsection{Supervised adaptation}

Existing self-explaining models such as SENN\cite{alvarez2018towards} is comprised of a concept network $g$, which is typically an autoencoder architecture to extract internal latent codes as concepts, as well as a relevance network $\theta$, which is a feedforward neural network that assigns a weight (i.e. relevance score) to each concept. The concepts and relevance scores are subsequently combined to perform downstream tasks using another network (i.e., aggregator). We defer to Appendix for more details on the complete architecture and all associated formulas. One paramount barrier for concepts in SENN-type networks to generalize is that the concepts are generated in an entirely unsupervised fashion which lacks sufficient guidance on how they should behave. In SCA, we propose to leverage concepts generated with SSCE from the source domain as initialization and proper supervision for target domain concept learning.

To perform supervised adaptation, we initialize the concept network ($g$) with weights from the SSCE encoder ($f_e(x)$) learned during the SSCE phase. To enforce that the concepts learned are not too dissimilar, we supervise training using a set of concept codes described in Section~\ref{sec:codebook}.

% Specifically, for source samples belonging to the same class, we compute the centroid of their concepts from SSCE as ground truth and impose a penalty on the concept network based on the discrepancy against the ground truth. We dub the computed centroid as ``codebook'' to reflect it is a reference for the target domain to refer to. Our design generates robust and domain invariant concepts that improve domain generalization, as shown in our empirical experiments. 



\subsubsection{Prototype Concept Codebook and Supervision Using Concept Codes}
\label{sec:codebook}
% \label{sec:supervision}


%% Interpretability - analysis
For each class in the training data, a small subset $\mathcal{S}_c$ of data belonging to a class $c$ is sampled from the training data. The associated concept codes of all samples in $\mathcal{S}_c$ are computed using $f_e$. Subsequently, a representative concept code for a class $c$ denoted by $\mathcal{C}_c$ is computed by averaging concept codes for all samples in $\mathcal{S}_c$ as in Equation~\ref{eq:rep-cc} and further stored in a concept codebook to be further utilized.
\begin{equation}
    \label{eq:rep-cc}
    \mathcal{C}_c = \frac{1}{|S_c|}\Sigma_{j}^{|S_c|} f_e(x^{c}_{j})
\end{equation}


% \jianhui{no label and no reference to this formula, currently too stand alone}

% Mathematically, the optimization can be formulated as:
% \begin{equation}
%     L_y(f(x), y) + \lambda L_\theta(f) + \xi L_h(x, \hat{x}) 
% \end{equation}

As robust concept codes have already been learned from SSCE, pre-trained information from the Concept Codebook computed in \ref{sec:codebook} can be used to aid in concept-learning in self-explaining models like SENN\cite{alvarez2018towards}. The model consists of two networks - a concept $g$ (Note that $f_e$ during inference is denoted by $g$) and relevance network $\theta$. The concepts and relevance scores are combined to perform downstream tasks using a feedforward network $a$ (aggregator). The entire network is trained end-to-end using a weighted sum of reconstruction loss ($\mathcal{L}_h$), classification loss ($\mathcal{L}_y$) and robustness loss ($\mathcal{L}_{\theta}$). For further details on the complete structure, please refer to Appendix. We utilize the concepts from the codebook to further supervise the unsupervised concept learning.
Mathematically, for a given class $c$ and concept code $\mathcal{C}_c$, the updated loss function of a self-explaining model can be written as:
% look at indexing in this:
\begin{equation}
    \label{eq:supervised-senn}
    L_y(a(x), y) + \lambda*L_\theta(a) + \xi*L_h(x, x) + \epsilon* l(g(x),\mathcal{C}_c) 
\end{equation}
where $l$ is a customized similarity measure and $L_y$, $L_\theta(g)$ and $L_h$ are the prediction, robustness and reconstruction loss, respectively. Supervision using concepts learned from SSCE forces the self-explainaing model to learn domain-invariant concepts for further downstream tasks.





